$\aleph_1$ and the modal $\mu$-calculus

For a regular cardinal $\kappa$, a formula of the modal $\mu$-calculus is $\kappa$-continuous in a variable x if, on every model, its interpretation as a unary function of x is monotone and preserves unions of $\kappa$-directed sets. We define the fragment $C_{\aleph_1}(x)$ of the modal $\mu$-calculus and prove that all the formulas in this fragment are $\aleph_1$-continuous. For each formula $\phi(x)$ of the modal $\mu$-calculus, we construct a formula $\psi(x) \in C_{\aleph_1 }(x)$ such that $\phi(x)$ is $\kappa$-continuous, for some $\kappa$, if and only if $\phi(x)$ is equivalent to $\psi(x)$. Consequently, we prove that (i) the problem whether a formula is $\kappa$-continuous for some $\kappa$ is decidable, (ii) up to equivalence, there are only two fragments determined by continuity at some regular cardinal: the fragment $C_{\aleph_0}(x)$ studied by Fontaine and the fragment $C_{\aleph_1}(x)$. We apply our considerations to the problem of characterizing closure ordinals of formulas of the modal $\mu$-calculus. An ordinal $\alpha$ is the closure ordinal of a formula $\phi(x)$ if its interpretation on every model converges to its least fixed-point in at most $\alpha$ steps and if there is a model where the convergence occurs exactly in $\alpha$ steps. We prove that $\omega_1$, the least uncountable ordinal, is such a closure ordinal. Moreover we prove that closure ordinals are closed under ordinal sum. Thus, any formal expression built from 0, 1, $\omega$, $\omega_1$ by using the binary operator symbol + gives rise to a closure ordinal.

==> macros.tex <==

\makeatletter
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\makeatother

% \RequirePackage[usenames]{xcolor}
\RequirePackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\RequirePackage{ifthen}
\RequirePackage{xspace}
\RequirePackage{amsmath,amsthm}
\RequirePackage{xspace,color}
% \RequirePackage{hyperref}
\RequirePackage{graphicx}
% \RequirePackage{enumitem}
\RequirePackage{nameref}
\RequirePackage{comment}


\newcommand{\MYparagraph}[1]{\par\smallskip\noindent\textbf{\emph{#1}}~}

\usepackage[normalem]{ulem}
\ifx\undefined\corrections
\newcommand{\correction}[3][None]{#3}
\newcommand{\rephrase}[2]{#2}
\else
\newcommand{\correction}[3][None]{\blue{#3}\footnote{Original :
    \red{#2}\\Comments : #1}}
\newcommand{\rephrase}[2]{\red{\sout{#1}} \blue{#2}}
\fi
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\let\GenerateWarning=\errmessage}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\TBC}{\red{TO BE COMPLETED}}
\newcommand{\LScomment}[1]{\textcolor{violet}{$\rangle\rangle$ LS : #1
    $\langle\langle$}}
\newcommand{\MGcomment}[1]{\textcolor{orange}{$\rangle\rangle$ MG : #1
    $\langle\langle$}}



\theoremstyle{plain}
% \newtheorem{proposition}{Proposition}
% \newtheorem{theorem}[proposition]{Theorem}
% \newtheorem{lemma}[proposition]{Lemma}
\newtheorem*{claim}{Claim}
\ifthenelse{\isundefined{\preprint}}{}{
  \newtheorem*{fact}{Fact}
  \newcommand{\titlecomment}[1]{\thanks{#1}}
}
% \newtheorem{corollary}[proposition]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[proposition]{Definition}
% \theoremstyle{remark}
% \newtheorem{remark}[proposition]{Remark}
% \newtheorem{example}[proposition]{Example}
% \newtheorem{problem}[proposition]{Problem}
% \newtheorem*{notation}{Notation}

\newcommand{\qedClaim}{\mbox{\hspace{1mm}}\hfill\mbox{$\Box$~\it{Claim.}}}
\newenvironment{proofofclaim}{\par\noindent{\it Proof of
    Claim.}}{
  \qedClaim \\ \par\noindent}
\newenvironment{proofofclaimNoQed}{\par\noindent{\it Proof of
    Claim.}}{
  \par\noindent}


\theoremstyle{Claim}
\newtheorem{Claim}{Claim}
\newenvironment{proofofclaim1}{\par\noindent{\it Proof of
    Claim~1.}}{
  \qed~\it{Claim~1}. \\ \par\noindent}
\newenvironment{proofofclaim2}{\par\noindent{\it Proof of
    Claim~2.}}{
  \qed~\it{Claim~2}. \\ \par\noindent}
\newenvironment{proofofclaim3}{\par\noindent{\it Proof of
    Claim~3.}}{
  \qed~\it{Claim~3}. \\ \par\noindent}

\newcommand{\new}[1]{\tilde{#1}} \newcommand{\card}{\mathrm{card}\,}
\newcommand{\set}[1]{\{\,#1 \,\}}
\newcommand{\sset}[1]{\{#1\}}
\newcommand{\rto}{\xrightarrow{\,\,}}
\newcommand{\kdirected}[1][$\kappa$]{#1-directed\xspace}
\newcommand{\kdirset}[1][$\kappa$]{\kdirected[#1] set\xspace}
\newcommand{\dirset}[1][$\kappa$]{\kdirset[#1]}
\newcommand{\ideal}{$\kappa$-ideal\xspace}
\newcommand{\continuous}[1][$\kappa$]{#1-continuous\xspace}
\newcommand{\kcontinuous}[1][$\kappa$]{\mbox{#1-continuous}\xspace}
\newcommand{\continuity}[1][$\kappa$]{#1-continuity\xspace}
\newcommand{\kcontinuity}[1][$\kappa$]{\mbox{#1-continuity}\xspace}
\newcommand{\ksmall}[1][$\kappa$]{#1-small\xspace}
\newcommand{\downset}[1]{\mbox{$\downarrow\!{#1}\,$}}
\newcommand{\Hartog}{\Omega}


\RequirePackage{amssymb}
\newcommand{\pos}[1][\;\;]{\langle #1 \rangle}
\newcommand{\nec}[1][\;\;]{[#1]}
\newcommand{\pmorphism}{$\mathrm{p}$-morphism\xspace}
\newcommand{\psubmodel}{$\mathrm{p}$-submodel\xspace}
\newcommand{\V}[1]{|#1|}


\newcommand{\bv}{\bigvee}
\newcommand{\Ik}{\mathcal{I}_{\kappa}}

\newcommand{\C}[1][1]{\mathcal{C}_{\aleph_{#1}}}
\newcommand{\CC}[1][\aleph_{1}]{\mathcal{C}_{#1}}
\newcommand{\T}{\mathcal{T}}

\newcommand{\trans}[1][]{R_{#1}}
\newcommand{\step}[1][\,]{\trans[#1]}

\newcommand{\N}{\mathbb{N}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Lmu}{\mathsf{L}_{\mu}}
\newcommand{\expanded}[1][$\kappa$]{#1-expanded\xspace}

\newcommand{\ie}{i.e.\xspace}
\newcommand{\K}{\ensuremath{\mathbf{K}}}
\newcommand{\five}{\text{\bf{5}}\xspace}
\newcommand{\Sfour}{\ensuremath{\mathbf{S}}\text{\bf{4}}\xspace}
\newcommand{\M}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\Ras}{\set{R_{a} \mid a \in \Act }}
\newcommand{\RM}{\set{R_{a}^{\M} \mid a \in \Act }}
\newcommand{\RN}{\set{R_{a}^{\NN} \mid a \in \Act }}

\newcommand{\negation}[1]{\overline{#1}}
\newcommand{\U}[1]{|#1|}
\newcommand{\clor}{\mathsf{cl}}
\newcommand{\closure}[2][]{\clor_{#1}(#2)}

\RequirePackage{stmaryrd}
\newcommand{\ldb}{\llbracket}
\newcommand{\rdb}{\rrbracket}

\newcommand{\eval}[2][\M]{\ldb #2 \rdb_{#1}}
\newcommand{\interpret}[2][\M]{|\!\!| \,#2 \,|\!\!|_{#1}}
\newcommand{\variant}[2][\M]{#1[#2]}
\newcommand{\evalN}[1]{\eval[\NN]{#1}}
  \newcommand{\evalMphi}[1]{\eval[\M\restr{\eval{\phi}}]{#1}}
\newcommand{\MUphi}{\M\restr{\eval{\Unv\chi}}}
\newcommand{\evalMUphi}[1]{\eval[\MUphi]{#1}}
\newcommand{\evalMzero}[1]{\eval[\M_{0}]{#1}}
\newcommand{\evalMone}[1]{\eval[\M_{1}]{#1}}

\newcommand{\flatten}[2][]{(#2)^{\flat #1}}
\newcommand{\flattenNp}[2][]{#2^{\flat #1}}

\newcommand{\lift}[2][x]{(#2)^{\sharp #1}}
\newcommand{\liftNp}[2][x]{#2^{\sharp #1}}
\newcommand{\lphi}{\liftNp{\phi}}
\newcommand{\mphin}[1]{{}_{_{#1}}}


\newcommand{\boxing}[2][]{\boxingNp[#1]{(#2)}}
\newcommand{\boxingNp}[2][]{#2^{\Box #1}}
\newcommand{\fphi}{\phi^{\flat}}
\newcommand{\subst}{[x/\x]}
\newcommand{\substp}{[\Const/\x]}
\newcommand{\CL}{\mathrm{CL}}
\ifthenelse{\isundefined{\CSL}}{
  \renewcommand{\boxed}[1]{\overline{#1}}
  \renewcommand{\Vec}[1]{\overline{#1}}
}{
  \renewcommand{\boxed}[1]{\overline{#1}}
  \renewcommand{\Vec}[1]{\overline{#1}}
}
\newcommand{\x}{\boxed{x}}
\newcommand{\y}{p}
\newcommand{\z}{q}
\newcommand{\tphi}{\tilde{\phi}}
\newcommand{\sigmaphi}{\sigma^{\phi}}
\newcommand{\sigmaphis}{\sigma^{\phi\cdot\substp}}
\newcommand{\sigmalphi}{\sigma^{\lphi}}
\newcommand{\restr}[1]{{}_{\restriction #1}}
\newcommand{\restrm}[1]{{}_{#1}}
\newcommand{\impl}{\rightarrow}
\newcommand{\tand}{\text{ and }}
\newcommand{\tor}{\text{ or }}
\newcommand{\tst}{\text{ s.t. }}
\newcommand{\timplies}{\text{ implies }}
\newcommand{\tiff}{\text{ iff }}

\renewcommand{\complement}[1]{{#1}^{\mathtt{c}}}
\newcommand{\substitute}[1]{[#1]}
\newcommand{\B}{\mathcal{B}}
\newcommand{\cS}{\complement{S}}

\newcommand{\nguarded}{boxed\xspace}
\newcommand{\Boxed}{boxed\xspace}
\newcommand{\good}{almost-good\xspace}
\newcommand{\agood}{almost-good\xspace}
\newcommand{\bad}{bad\xspace}
\newcommand{\vbad}{very-\bad}
\newcommand{\nsbad}{slightly-\bad}
\newcommand{\linear}{linearly-quantified\xspace}
\newcommand{\wnamed}{well-named\xspace}
\newcommand{\Wnamed}{Well-named\xspace}

\newcommand{\f}{\mathsf{f}}
\newcommand{\MS}{\M\restr{S}}
\newcommand{\McS}{\M\restr{\complement{S}}}
\newcommand{\evalMS}[1]{\eval[\MS]{#1}}
\newcommand{\evalMcS}[1]{\eval[\McS]{#1}}

\newcommand{\Unv}{\nec[\,\mathcal{U}\,]}
\newcommand{\Master}{\nec[\,\mathcal{U}\,]}
\newcommand{\na}{\new{a}}

\newcommand{\multimodal}{multimodal\xspace}
\newcommand{\UM}{\U{\M}}
\newcommand{\UF}{\U{\FF}}

\newcommand{\fcheck}[2][]{(#2){\check{}}\,}
\newcommand{\loperator}{@\,}

\newcommand{\Act}{Act}

\newcommand{\forces}{\Vdash}
\newcommand{\MO}{\M_{\omega_1}}
\newcommand{\simul}[1]{#1^{sim}}
\newcommand{\wcirc}[1]{#1^{\circ}}
\newcommand{\circfunction}{\wcirc{(_{-})}}


\newcommand{\pair}[2]{#1 \,\rightarrowtail \,#2}

\newcommand{\evalF}[2][]{
  \ifthenelse{\equal{#1}{}}
  {\eval[\FF_{v}\substitute{\pair{\y}{G}}]{#2}}
  {\eval[\FF_{v}\substitute{\pair{\y}{G},#1}]{#2}}
}
\newcommand{\evalG}[2][]{
  \ifthenelse{\equal{#1}{}}
  {\eval[\GG_{\pi\circ v}]{#2}}
  {\eval[\GG_{\pi\circ v}\substitute{#1}]{#2}}
}


\newcommand{\lfp}{\mathtt{lfp}}
\newcommand{\gfp}{\mathtt{gfp}}

\newcommand{\acceptable}{acceptable\xspace}
\newcommand{\chiacceptable}{$\chi$-acceptable\xspace}
\newcommand{\iso}{\simeq}

\RequirePackage[all]{xy}

\newcommand{\BLABLA}{\blue{BLA BLA BLA \ldots }}

\newcommand{\Ord}{\mathrm{Ord}}
\newcommand{\OrdLmu}{\mathrm{Ord}(\Lmu)}

\newcommand{\complex}[1]{{#1}^{\sharp}}
\newcommand{\tr}[1][\Psi]{\mathtt{tr}^{#1}}
\newcommand{\trp}{\tr[]}
\newcommand{\trsim}[1]{#1^{\mathtt{sim}}}

\newcommand{\rightside}[2][5mm]{\makebox[#1][l]{${\displaystyle #2}$}}
\newcommand{\smallRHS}[2][5mm]{\makebox[#1][l]{${\displaystyle #2}$}}
\newcommand{\smallLHS}[2][5mm]{\makebox[#1][l]{${\displaystyle #2}$}}
\newcommand{\Pref}{\mathtt{Pre}}
\newcommand{\Post}{\mathtt{Pos}}
\newcommand{\tuple}[1]{\langle#1\rangle}

\newcommand{\phiU}{\trp(\phi_{1})}
\newcommand{\psiN}{\psi\mphin{\NN}}
\newcommand{\phiNz}{\phi\mphin{\NN_{0}}}
\newcommand{\phiNu}{\phi\mphin{\NN_{1}}}

\newcommand{\myrule}[1][14pt]{\rule{0pt}{#1}}

\newcommand{\FP}{fixed-point\xspace}
\newcommand{\LFP}{least fixed-point\xspace}
\newcommand{\GFP}{greatest fixed-point\xspace}
\newcommand{\GGFP}{Greatest fixed-point\xspace}


\newcommand{\PHI}{\Phi}

\newcommand{\proofs}[1]{Proofs from Section~\ref{#1}, \nameref{#1}}

% \newtheorem{lemma*}{Lemma}
% \newtheorem{proposition*}{Proposition}

\newenvironment{myfact}{\par\noindent\textbf{Fact.}\it}{\par\noindent}
\newcommand{\phiM}{\phi_{\M}}
\newcommand{\psiM}{\psi_{\M}}
\newcommand{\eset}{(\emptyset)}
\newcommand{\DELTA}{\nabla}
\newcommand{\qedExample}[1]{\hfill\mbox{$\Box$~\it{Example~\ref{#1}.}}}
\newcommand{\MYendexample}[1]{\qedExample{#1}}

\newcommand{\refines}{\ll}

\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother

\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}
\newcommand{\bigcupdot}{\charfusion[\mathbin]{\bigcup}{\cdot}}
\newcommand{\dcup}{\mathbin{\dot{\cup}}}
\newcommand{\dunion}{\cupdot}
\newcommand{\dUnion}{\bigcupdot}

\newcommand{\universal}{master\xspace}
\newcommand{\master}{master\xspace}
\newcommand{\ENDOFPROOF}[1][Proposition]{This concludes the proof of
  #1.\xspace}

\newcommand{\sttr}[1]{ST_{y}(#1)}

\newcommand{\spacelesstext}[1]{\makebox[3mm][l]{#1}}
\newcommand{\eqdef}{:=}

\newcommand{\Const}{\gamma}
\newcommand{\myldots}{\;\ldots\;}
\newcommand{\pit}{p_{0}}
\newcommand{\clK}{\mathcal{K}}
\newcommand{\Lower}{lower\xspace}
\newcommand{\Upper}{upper\xspace}
\newcommand{\Ladjoint}{\Lower adjoint\xspace}
\newcommand{\Uadjoint}{\Upper adjoint\xspace}
\newcommand{\Czarnecki}{Czarnecki\xspace}
\makeatletter
\define@key{Gin}{resolution}{\pdfimageresolution=#1\relax}
\makeatother


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "0.tex"
%%% End:

